A Robust CNN Framework with Dual Feedback Feature Accumulation for Detecting Pneumonia Opacity from Chest X-ray Images

Pneumonia is one of the most acute respiratory diseases having remarkably high prevalence and mortality rate. Chest X-ray (CXR) has been widely utilized for the diagnosis of this disease owing to its availability, diagnostic speed and accuracy. However, even for an expert radiologist, it is quite challenging to readily determine pneumonia opacity by examining CXRs. Therefore, this study has been structured to automate the pneumonia detection process by introducing a robust deep learning framework. The proposed network comprises of Process Convolution (Pro_Conv) blocks for feature accumulation inside Dual Feedback (DF) blocks to propagate the feature maps towards a viable detection. Experimental analysis showcase: (1) the proposed network proficiently distinguishes between normal and pneumonia opacity containing CXRs with the mean accuracy, sensitivity and specificity of 97.78%, 98.84% and 95.04%, respectively; (2) the network is constructed with significantly low parameters than the traditional ImageNets to reduce memory consumption for deployment in memory constrained mobile platforms; (3) the trade-off between accuracy and number of parameters of the model outperforms the considered classical networks by a remarkable margin; and (4) the false-negatives are lower than the false-positives (both of which are low in count) which prove the model's low-fatality prediction. Hence, the proposed network can be deployed for a rapid screening of pneumonia and can act as a great assistive tool for the radiologists in the diagnosis process.

==> algorithm2e/doc/algorithm2e_ex01.tex <==
\SetAlgoVlined
\eIf{cond1}{
  a line\;
  a line\;
}{
  another line\;
  another line\;
}


==> algorithm2e/doc/algorithm2e_ex02.tex <==
\SetAlgoNoLine
\If{cond2}{
  second if\;
  second if\;
}


==> algorithm2e/doc/algorithm2e_ex03.tex <==
\lIf{cond3}{ another example}
\Else{
  a block\;
  a block\;
}


==> algorithm2e/doc/algorithm2e_ex04.tex <==
\lIf{cond4}{ok} \lElse{wrong}
\leIf{cond4}{ok}{wrong}


==> algorithm2e/doc/algorithm2e_ex05.tex <==
\SetAlgoVlined
\lIf{cond5}{cond5 true}
\uElseIf{cond51}{
  cond 5 false\;
  but cond51 true\;
}
\ElseIf{}{
  all is wrong\;
  \Return result52\;
}


==> algorithm2e/doc/algorithm2e_ex06.tex <==
\SetAlgoLined
\uIf{cond6}{
  cond6 is ok\;
  always ok\;
}
\uElseIf{cond62}{
  choose result62\;
  \Return result62\;
}
\Else{
  all is wrong\;
  do something else\;
}


==> algorithm2e/doc/algorithm2e_ex07.tex <==
Let's have a look at what we can do
with if-then-else and side comments\;
\eIf{if-then-else test}{
  no comment here\;
  neither in then\;
}{
  nor in else\;
}
\eIf(\tcc*[f]{then comment}){test}{
  then with a comment\;
}(\tcc*[f]{comment in else})
{
  here we are in else\;
}
\eIf(\tcc*[f]{then comment}){test}{
  again a comment in then\;
}{
  but not in else\;
}
\eIf{if-then-else test}{
  this time, no comment in then\;
}(\tcc*[f]{else comment})
{
  but one comment in else\;
}
Let's try with other if possibilities\;
\lIf(\tcc*[h]{lif comment}){test}{text}
\uIf(\tcc*[f]{uif comment}){test}{
  then text\;
}
\uElseIf(\tcc*[f]{comment}){test}{
  elseif text\;
}
\lElseIf(\tcc*[h]{comment}){test}{text}
\lElse(\tcc*[f]{comment}){text}


==> algorithm2e/doc/algorithm2e_exAlgoDisjdecomp.tex <==
\IncMargin{1em}
\begin{algorithm}
  \SetKwData{Left}{left}\SetKwData{This}{this}\SetKwData{Up}{up}
  \SetKwFunction{Union}{Union}\SetKwFunction{FindCompress}{FindCompress}
  \SetKwInOut{Input}{input}\SetKwInOut{Output}{output}

  \Input{A bitmap $Im$ of size $w\times l$}
  \Output{A partition of the bitmap}
  \BlankLine
  \emph{special treatment of the first line}\;
  \For{$i\leftarrow 2$ \KwTo $l$}{
    \emph{special treatment of the first element of line $i$}\;
    \For{$j\leftarrow 2$ \KwTo $w$}{\label{forins}
      \Left$\leftarrow$ \FindCompress{$Im[i,j-1]$}\;
      \Up$\leftarrow$ \FindCompress{$Im[i-1,]$}\;
      \This$\leftarrow$ \FindCompress{$Im[i,j]$}\;
      \If(\tcp*[h]{O(\Left,\This)==1}){\Left compatible with \This}{\label{lt}
        \lIf{\Left $<$ \This}{\Union{\Left,\This}}
        \lElse{\Union{\This,\Left}}
      }
      \If(\tcp*[f]{O(\Up,\This)==1}){\Up compatible with \This}{\label{ut}
        \lIf{\Up $<$ \This}{\Union{\Up,\This}}
        \tcp{\This is put under \Up to keep tree as flat as possible}\label{cmt}
        \lElse{\Union{\This,\Up}}\tcp*[h]{\This linked to \Up}\label{lelse}
      }
    }
    \lForEach{element $e$ of the line $i$}{\FindCompress{p}}
  }
  \caption{disjoint decomposition}\label{algo_disjdecomp}
\end{algorithm}\DecMargin{1em}

==> algorithm2e/doc/algorithm2e_exIR.tex <==
\begin{algorithm}
\DontPrintSemicolon
\KwData{$G=(X,U)$ such that $G^{tc}$ is an order.}
\KwResult{$G'=(X,V)$ with $V\subseteq U$ such that $G'^{tc}$ is an
interval order.}
\Begin{
  $V \longleftarrow U$\;
  $S \longleftarrow \emptyset$\; 
  \For{$x\in X$}{ 
    $NbSuccInS(x) \longleftarrow 0$\;
    $NbPredInMin(x) \longleftarrow 0$\;
    $NbPredNotInMin(x) \longleftarrow |ImPred(x)|$\;
    }
  \For{$x \in X$}{
    \If{$NbPredInMin(x) = 0$ {\bf and} $NbPredNotInMin(x) = 0$}{
      $AppendToMin(x)$}
    } 
    \nl\While{$S \neq \emptyset$}{\label{InRes1}
    \nlset{REM} remove $x$ from the list of $T$ of maximal index\;\label{InResR}
    \lnl{InRes2}\While{$|S \cap  ImSucc(x)| \neq |S|$}{ 
      \For{$ y \in  S-ImSucc(x)$}{
        \{ remove from $V$ all the arcs $zy$ : \}\;
        \For{$z \in  ImPred(y) \cap  Min$}{
          remove the arc $zy$ from $V$\;
          $NbSuccInS(z) \longleftarrow NbSuccInS(z) - 1$\;
          move $z$ in $T$ to the list preceding its present list\;
          \{i.e. If $z \in T[k]$, move $z$ from $T[k]$ to 
           $T[k-1]$\}\;
          }
        $NbPredInMin(y) \longleftarrow 0$\;
        $NbPredNotInMin(y) \longleftarrow 0$\;
        $S \longleftarrow S - \{y\}$\;
        $AppendToMin(y)$\;
        }
      }
    $RemoveFromMin(x)$\;
    }
  }  
\caption{IntervalRestriction\label{IR}}
\end{algorithm}


==> algorithm2e/doc/algorithm2e_exProg.tex <==
\SetAlgoLined
\SetKwProg{Fn}{Function}{ is}{end}
\Fn{afunc(i: int) : int}{return 0\;}  

\SetKwProg{Def}{def}{:}{}
\Def{afunc(i: int)}{return 0\;}

==> algorithm2e/doc/algorithm2e_exfor.tex <==
\SetAlgoLined
\ForAll{elements of $S_1$}{
  remove an element e from $S_1$\;
  put e in the set $S_2$\;
  }
\lFor{i=1 \emph{\KwTo}max}{mark i}\;
\ForEach{$e$ in the set}{
  put $e$ in ${\cal E}$\;
  mark $e$\;
}


==> algorithm2e/doc/algorithm2e_exgeneric.tex <==
\Fn(\tcc*[h]{algorithm as a recursive function}){\FRecurs{some args}}{
  \KwData{Some input data\\these inputs can be displayed on several lines and one 
    input can be wider than line's width.}
  \KwResult{Same for output data}
  \tcc{this is a comment to tell you that we will now really start code}
  \If(\tcc*[h]{a simple if but with a comment on the same line}){this is true}{
    we do that, else nothing\;
    \tcc{we will include other if so you can see this is possible}
    \eIf{we agree that}{
      we do that\;
    }{
      else we will do a more complicated if using else if\;
      \uIf{this first condition is true}{
        we do that\;
      }
      \uElseIf{this other condition is true}{
        this is done\tcc*[r]{else if}
      }
      \Else{
        in other case, we do this\tcc*[r]{else}
      }
    }
  }
  \tcc{now loops}
  \For{\forcond}{
    a for loop\;
  }
  \While{$i<n$}{
    a while loop including a repeat--until loop\;
    \Repeat{this end condition}{
      do this things\;
    }
  }
  They are many other possibilities and customization possible that you have to
  discover by reading the documentation.
}


==> algorithm2e/doc/algorithm2e_exgeneric2.tex <==
\Fn(\tcc*[h]{algorithm as a recursive function}){\FRecurs{some args}}{
  \KwData{Some input data}
  \KwResult{Same for output data}
  \If(\tcc*[h]{a simple if but with a comment on the same line}){this is true}{
    we do that, else nothing\;
    \lIf{we agree that}{we do that}
    \Else{
      \lIf{this first condition is true}{we do that}
      \lElseIf(\tcc*[h]{else if}){this other condition is true}{this is done}
      \lElse(\tcc*[h]{else}){in other case, we do this}
    }
  }
  \lFor{\forcond}{a for loop}
  \While{$i<n$}{
    a while loop including a repeat--until loop\;
    \lRepeat(\tcc*[h]{a comment}){this end condition}{do this things}
  }
  They are many other possibilities and customization possible that you have to
  discover by reading the documentation.
}


==> algorithm2e/doc/algorithm2e_exnlsty.tex <==
\SetNlSty{texttt}{[}{]}
\SetAlgoNlRelativeSize{0}
\SetNlSkip{0em}
\nl\KwIn{input data}
\nl\KwOut{output data}
\nl\tcc{a comment line in C-style}
\nl\Repeat{\nl$e<\tau$}{
  \nl$f_n\leftarrow Y_1$\;
  \nl$f_{n+1}\leftarrow f_n\times f_{n-1}$\;
  \nl$e\leftarrow \frac{f_n}{2}$\;
}
\nl\KwRet{$e$}

==> algorithm2e/doc/algorithm2e_exrepeat.tex <==
\Repeat{this stop condition}{
  the text of the loop\;
  another line\;
  always in the loop\;
  }
\lRepeat{stop}{a one line loop}


==> algorithm2e/doc/algorithm2e_exswitch.tex <==
\Switch{the value of T}{
  \uCase{a value}{
    do this\;
    do that\;
  }
  \lCase{another value}{one line}
  \Case{last value}{
    do this\;
    break\;
  }
  \Other{
    for the other values\;
    do that\;
  }
}


==> cite/README <==
This directory contains four .sty files that are mutually compatible,
but (mostly) independent:

cite.sty       Compressed, sorted lists of numerical citations: [8,11-16]
               with many options for controlling the formatting.

overcite.sty   like \usepackage[superscript]{cite}

drftcite.sty   Print the tags instead of the numbers for \cite and \bibitem.

chapterbib.sty Do multiple bibliographies--one for each \include file.

The user manuals for cite and chapterbib are LaTeX files cite.ltx
and chapterbib.ltx, and already typeset pdf versions.

They are all released under a very simple permissive license in
the MIT/BSD style:  They may be freely used, transmitted, reproduced, 
or modified provided that the copyright and permission notice is 
left intact.



Donald Arseneau                         asnd@triumf.ca


==> hyperref/abbr.tex <==
\abbrdef{``}{\texorpdfstring{``}{\flqq}}
\abbrdef{''}{\texorpdfstring{''}{\frqq}}
\abbrdef{acroread}{\Program{AcrobatReader}}
\abbrdef{aux}{\File{.aux}}
\abbrdef{eg}{e.\,g\mbox{.}}
\abbrdef{gdi}{general document information}
\abbrdef{gs}{\Program{ghost\-script}}
\abbrdef{hyperref}{\Package{hy\-per\-ref}}
\abbrdef{hypbmsec}{\Package{hypbmsec}}
\abbrdef{ind}{\hbox{\texttt{ \ }}}
\abbrdef{isolatin1}{ISOLatin1}
\abbrdef{latex}{\LaTeX}
\abbrdef{latexe}{\texorpdfstring{\LaTeXe}{LaTeX2e}}
\abbrdef{mediabox}{/MediaBox}
\abbrdef{PD1}{PD1}
\abbrdef{pdf}{PDF}
\abbrdef{pdfdocencoding}{PDFDocEncoding}
\abbrdef{pdffile}{pdf file}
\abbrdef{pdfinfo}{\Program{pdfinfo}}
\abbrdef{pdfspec}{*pdf* specification}
\abbrdef{pdfstringdef}{\cms{pdfstringdef}}
\abbrdef{pdftex}{\Program{\pdfTeX}}
\abbrdef{perlscript}{perl script}
\abbrdef{plain}{plain}
\abbrdef{plaintex}{*plain*-*tex*}
\abbrdef{postscript}{PostScript}
\abbrdef{PU}{PU}
\abbrdef{sectioning}{section} % section?
\abbrdef{Sectioning}{Section}
\abbrdef{tex}{\TeX}
\abbrdef{texfile}{*tex* file}
\abbrdef{thumbpdf}{\Package{thumb\-pdf}}
\abbrdef{thumbpdf.pl}{\File{thumbpdf.pl}}
\abbrdef{toc}{\File{.toc}}
\abbrdef{unicode}{Unicode}
\abbrdef{winansiencoding}{WinAnsiEncoding}
\endinput


==> hyperref/docinfo.tex <==
\foilhead[-\baselineskip]{General Document Information}

%\begin{Nav}{\NavInfo\NavBack}%
\begin{Nav}{\NavInfo}%
  \newcommand{\tit}[1]{%
    \multicolumn{2}{@{}l@{}}{\textbf{#1}}\\[0.5ex]%
  }
  \newcommand{\longentry}[1]{%
    \multicolumn{2}{@{}l@{}}{#1}%
  }
  \noindent
  Application: search engines.

  \noindent
  \begin{minipage}[t]{.55\linewidth}
    \begin{tabular}[t]{@{}l>{\tt}l@{}}
    \tit{\hypertarget{info}{*hyperref* options:}}%
    Title:&\Blue{pdftitle}\\
    Subject:&\Blue{pdfsubject}\\
    Author:&\Blue{pdfauthor}\\
    Keywords:&\Blue{pdfkeywords}\\
    Creator:&\Blue{pdfcreator}\\
    Producer:&\Blue{pdfproducer}
    \end{tabular}
  \end{minipage}%
  \begin{minipage}[t]{.45\linewidth}
    \begin{tabular}[t]{@{}ll@{}}
      \tit{Times:}%
      Created:&\Green{/CreationDate}\\
      Modificated:&\Green{/ModDate}\\[1ex]
      \tit{Informations:}%
      \longentry{File name, file size}\\
      \longentry{*pdf* version}\\
      \longentry{Optimized(linearized)}
    \end{tabular}
  \end{minipage}

  \subfoilhead{Setting\texorpdfstring{ the general document information}{}}
  \begin{smallpar}\hypertarget{infoanw}{}%
  \noindent
  \Code{\cms{usepackage}\{hyperref\}}\par
  \vspace{-\parskip}
  \catcode`\^^M=5
  \verbatiminput{pdfinfo}
  \end{smallpar}
  \newpage

\end{Nav}


\iffalse
\begingroup
  \makeatletter
  \def\hyper@anchorstart#1\hyper@anchorend{}%
  \pdfbookmark[1]{\file{hyperref} options}{optinfo}
\endgroup
\fi

\endinput


==> hyperref/encoding.tex <==
\clearpage
\pdfbookmark[0]{Encodings}{enc}

\begingroup
\hypersetup{bookmarksopenlevel=2}


\subfoilhead[-\baselineskip]{Font encoding mechanism%
  \texorpdfstring{}{ of \abbr{latexe}}}

\noindent
\begin{tabular}{@{}l@{ }l@{ $\Rightarrow$ }l@{}}
plain-\TeX:& \code[green]<\ss>\ = \code[blue]<\char"19>&\Red{\ss}\\[1ex]
\LaTeXe:
  & \code<\fontencoding{OT1}\selectfont\char"19>&\Red{\ss}\\
  & \code<\fontencoding {T1}\selectfont\char"19>&\Red{\i}\\[0.5ex]
  & \code<\ss>\ = \code[blue]<\OT1-cmd \ss > \code[green]<\OT1\ss>&\Red{\ss}
\end{tabular}

\noindent
The font slot positions depend on the encoding:\\
\phantom{plain-\TeX: }\code[green]<\OT1\ss>\ = \code<\char"19>\\
\phantom{plain-\TeX: }\code[green]<\T1\ss>\phantom{\code<O>} =
  \code<\char"FF>\\
\phantom{plain-\TeX: }\code[green]<\?\ss>\phantom{\code<OT>} =
  \code<\UseTextSymbol{OT1}\ss>

%\begin{smallpar}
  \noindent
  \code<\> \code[blue]<OT1\ss>\ =
  \code<\csname > \code[blue]<OT1> \code<\string> \code[blue]<\ss>
    \code<\endcsname>
%\end{smallpar}


\subfoilhead[-\baselineskip]{PD1 encoding%
  \texorpdfstring{ (\abbr{pdfdocencoding})}{}}

\begin{itemize}
\def\1{\code[red]}%
\def\2{\code[blue]}\def\3{\Blue}%
\def\4#1{\Green{#1}\,=\,}%
\def\5{\Green}
\item Most names: \1<\text>%
    \3{\textsl{\textless glyph name\textgreater}}\\
    Examples:\quad
  \begin{tabular}[t]{@{}c@{\,=\,}l@{,\quad}c@{\,=\,}l@{}}
    \5\textregistered&\1<\text>\2<registered>&
    \5\textasciitilde&\1<\text>\2<asciitilde>
  \end{tabular}
\item Traditional *tex* and *latex* names.\\
    Examples:\quad
    \4\AE\2<\AE>,\quad
    \4\ss\2<\ss>
\item Accented characters.\\
    Examples:\quad
    \4{\"U}\2<\"U>,\quad
    \4{\c c}\2<\c c>,\quad
    \4{\r A}\2<\r A>~($\Leftarrow$\,\1<\AA>)
\item Escape octal sequences are the result:
%  \2<\textmu>\ (\Green{$\mu$}) $\Rightarrow$ \1<\265>
%  \2<\guillemotleft>\ (\Green{\guillemotleft}) $\Rightarrow$ \1<\253>
  \2<\textmu>\,$\Rightarrow$\,\1<\265>
\end{itemize}


\subfoilhead[-1.5\baselineskip]{PU encoding%
  \texorpdfstring{ (\abbr{unicode})}{}}

\begin{itemize}
\item[\frownie] Characters having catcodes 11 (letter) and 12 (other):\\
Checking each token, high memory and time consumption.
\item[\frownie] Ligatures: same as above.
\item[\frownie] Direct commands:\\
  Easier to implement, but each command must be redefined each time.
\item[\smiley] Commands of *latexe*'s fontencoding mechanism:\\
  Smallest memory consumption and fastest method.\\
  This method is used by package *hyperref*.
\end{itemize}


\subsubfoilhead[-\baselineskip]{Examples of \abbr{unicode} bookmarks}

\begingroup
\def\top#1{\vtop{\vskip0pt\hbox{#1}}}
\def\use#1{\top{\includegraphics[scale=1.2]{u0#1}}}
\centering
\begin{tabular}{@{}ll@{}}
\Blue{Greek}:&\Blue{Cyrillic}:\\
\use{3}&\use{4}\\
\end{tabular}
\par
\endgroup

\endgroup
\endinput


==> hyperref/ende.tex <==
\clearpage
\pdfbookmark[0]{Ende}{ende}

\subfoilhead[-1.5\baselineskip]{Zusammenfassung}
\begin{itemize}
  \item \Red{Dokumenteninformation}:
    \begin{itemize}
      \item \file{hyperref}-Optionen in \code[blue]<\hypersetup>.
    \end{itemize}
  \item \Red{Lesezeichen}:
    \begin{itemize}
      \item Vorsicht wegen fehlender Magenverarbeitung
      \item Vieles durch \code[blue]<hyperref.sty>\ automatisiert.
      \item Zusatzpaket \code[blue]<hypbmsec.sty>
      \item Besondere Effekte erfordern "`low level"'-Eingriffe.
    \end{itemize}
  \item \Red{Thumbnails}:
    \begin{itemize}
      \item
      Einfache Benutzerschnittstelle mit \code[blue]<thumbpdf>.
    \end{itemize}
\end{itemize}


\subfoilhead[-\baselineskip]{Bezugsquellen}

\begin{smallpar}
\pdfadjustspacing=1
\noindent
\begingroup
\def\it{\textbullet}%
\def\sep{1ex}%
\begin{tabularx}{\linewidth}{@{}l@{ }X@{}}
  \it&\Blue{PDF-Spezifikation}:\hfill
\url{http://www.adobe.com/supportservice/devrelations/PDFS/TN/PDFSPEC.PDF}\\[\sep]
  \it&\Blue{pdf\TeX}: \url{http://www.tug.org/applications/pdftex/}\\
  &Win32: \url{ftp://ftp.ese-metz.fr/pub/TeX/win32-beta/}\\
  &Dokumantation: \url{http://www.pragma-ade.nl/pdftex.htm}\\[\sep]
  \it&\Blue{hyperref}, \Blue{pd1enc.def}, \Blue{hyparen.sty}:
\url{ftp://ftp.dante.de/tex-archive/macros/latex/contrib/supported/hyperref/}\\[\sep]
  \it&\Blue{hypbmsec}: Noch per E-Mail, CTAN geplant.\\[\sep]
  \it&\Blue{thumbpdf}:\hfill
\url{ftp://ftp.dante.de/tex-archive/macros/pdftex/thumbpdf/}\\[\sep]
  \it&\Blue{ghostscript}:
\url{http://www.cs.wisc.edu/~ghost/} oder\\&
\url{http://ftp.dante.de/tex-archive/support/ghostscript/aladdin/}
\end{tabularx}
\endgroup
\end{smallpar}

\rightfooter{%
  \ifprint
  \else
    \NavFull\NavSep\NavPrev\NavSep\NavQuit
  \fi
}


==> hyperref/eurobm99.tex <==
%\includeonly{title,docinfo,strings,encoding,psd,hyperref,replace,pdfextra,thumb,summary,links,appendix}
%\includeonly{hyperref}

\begin{document}
\catcode`\*=\active
\include{title}
\include{docinfo}
\include{strings}
\include{encoding}
\include{psd}
\include{hyperref}
\include{replace}
\include{pdfextra}
\include{thumb}
\include{summary}
\include{links}
\include{appendix}
\end{document}


==> hyperref/fdl.tex <==
% This file is a chapter.  It must be included in a larger document to work
% properly.

\chapter{GNU Free Documentation License}

Version 1.2, November 2002


 Copyright \copyright\ 2000,2001,2002  Free Software Foundation, Inc.\\
     59 Temple Place, Suite 330, Boston, MA  02111-1307  USA\\
 Everyone is permitted to copy and distribute verbatim copies
 of this license document, but changing it is not allowed.


\section*{PREAMBLE}

The purpose of this License is to make a manual, textbook, or other
functional and useful document ``free'' in the sense of freedom: to
assure everyone the effective freedom to copy and redistribute it,
with or without modifying it, either commercially or noncommercially.
Secondarily, this License preserves for the author and publisher a way
to get credit for their work, while not being considered responsible
for modifications made by others.

This License is a kind of ``copyleft'', which means that derivative
works of the document must themselves be free in the same sense.  It
complements the GNU General Public License, which is a copyleft
license designed for free software.

We have designed this License in order to use it for manuals for free
software, because free software needs free documentation: a free
program should come with manuals providing the same freedoms that the
software does.  But this License is not limited to software manuals;
it can be used for any textual work, regardless of subject matter or
whether it is published as a printed book.  We recommend this License
principally for works whose purpose is instruction or reference.


\section{APPLICABILITY AND DEFINITIONS}
\label{applicability}

This License applies to any manual or other work, in any medium, that
contains a notice placed by the copyright holder saying it can be
distributed under the terms of this License.  Such a notice grants a
world-wide, royalty-free license, unlimited in duration, to use that
work under the conditions stated herein.  The ``Document'', below,
refers to any such manual or work.  Any member of the public is a
licensee, and is addressed as ``you''.  You accept the license if you
copy, modify or distribute the work in a way requiring permission
under copyright law.

A ``Modified Version'' of the Document means any work containing the
Document or a portion of it, either copied verbatim, or with
modifications and/or translated into another language.

A ``Secondary Section'' is a named appendix or a front-matter section of
the Document that deals exclusively with the relationship of the
publishers or authors of the Document to the Document's overall subject
(or to related matters) and contains nothing that could fall directly
within that overall subject.  (Thus, if the Document is in part a
textbook of mathematics, a Secondary Section may not explain any
mathematics.)  The relationship could be a matter of historical
connection with the subject or with related matters, or of legal,
commercial, philosophical, ethical or political position regarding
them.

The ``Invariant Sections'' are certain Secondary Sections whose titles
are designated, as being those of Invariant Sections, in the notice
that says that the Document is released under this License.  If a
section does not fit the above definition of Secondary then it is not
allowed to be designated as Invariant.  The Document may contain zero
Invariant Sections.  If the Document does not identify any Invariant
Sections then there are none.

The ``Cover Texts'' are certain short passages of text that are listed,
as Front-Cover Texts or Back-Cover Texts, in the notice that says that
the Document is released under this License.  A Front-Cover Text may
be at most 5 words, and a Back-Cover Text may be at most 25 words.

A ``Transparent'' copy of the Document means a machine-readable copy,
represented in a format whose specification is available to the
general public, that is suitable for revising the document
straightforwardly with generic text editors or (for images composed of
pixels) generic paint programs or (for drawings) some widely available
drawing editor, and that is suitable for input to text formatters or
for automatic translation to a variety of formats suitable for input
to text formatters.  A copy made in an otherwise Transparent file
format whose markup, or absence of markup, has been arranged to thwart
or discourage subsequent modification by readers is not Transparent.
An image format is not Transparent if used for any substantial amount
of text.  A copy that is not ``Transparent'' is called ``Opaque''.

Examples of suitable formats for Transparent copies include plain
ASCII without markup, Texinfo input format, \LaTeX\ input format, SGML
or XML using a publicly available DTD, and standard-conforming simple
HTML, PostScript or PDF designed for human modification.  Examples of
transparent image formats include PNG, XCF and JPG.  Opaque formats
include proprietary formats that can be read and edited only by
proprietary word processors, SGML or XML for which the DTD and/or
processing tools are not generally available, and the
machine-generated HTML, PostScript or PDF produced by some word
processors for output purposes only.

The ``Title Page'' means, for a printed book, the title page itself,
plus such following pages as are needed to hold, legibly, the material
this License requires to appear in the title page.  For works in
formats which do not have any title page as such, ``Title Page'' means
the text near the most prominent appearance of the work's title,
preceding the beginning of the body of the text.

A section ``Entitled XYZ'' means a named subunit of the Document whose
title either is precisely XYZ or contains XYZ in parentheses following
text that translates XYZ in another language.  (Here XYZ stands for a
specific section name mentioned below, such as ``Acknowledgements'',
``Dedications'', ``Endorsements'', or ``History''.)  To ``Preserve the Title''
of such a section when you modify the Document means that it remains a
section ``Entitled XYZ'' according to this definition.

The Document may include Warranty Disclaimers next to the notice which
states that this License applies to the Document.  These Warranty
Disclaimers are considered to be included by reference in this
License, but only as regards disclaiming warranties: any other
implication that these Warranty Disclaimers may have is void and has
no effect on the meaning of this License.


\section{VERBATIM COPYING}
\label{verbatim}

You may copy and distribute the Document in any medium, either
commercially or noncommercially, provided that this License, the
copyright notices, and the license notice saying this License applies
to the Document are reproduced in all copies, and that you add no other
conditions whatsoever to those of this License.  You may not use
technical measures to obstruct or control the reading or further
copying of the copies you make or distribute.  However, you may accept
compensation in exchange for copies.  If you distribute a large enough
number of copies you must also follow the conditions in
section~\ref{copying}.

You may also lend copies, under the same conditions stated above, and
you may publicly display copies.


\section{COPYING IN QUANTITY}
\label{copying}

If you publish printed copies (or copies in media that commonly have
printed covers) of the Document, numbering more than 100, and the
Document's license notice requires Cover Texts, you must enclose the
copies in covers that carry, clearly and legibly, all these Cover
Texts: Front-Cover Texts on the front cover, and Back-Cover Texts on
the back cover.  Both covers must also clearly and legibly identify
you as the publisher of these copies.  The front cover must present
the full title with all words of the title equally prominent and
visible.  You may add other material on the covers in addition.
Copying with changes limited to the covers, as long as they preserve
the title of the Document and satisfy these conditions, can be treated
as verbatim copying in other respects.

If the required texts for either cover are too voluminous to fit
legibly, you should put the first ones listed (as many as fit
reasonably) on the actual cover, and continue the rest onto adjacent
pages.

If you publish or distribute Opaque copies of the Document numbering
more than 100, you must either include a machine-readable Transparent
copy along with each Opaque copy, or state in or with each Opaque copy
a computer-network location from which the general network-using
public has access to download using public-standard network protocols
a complete Transparent copy of the Document, free of added material.
If you use the latter option, you must take reasonably prudent steps,
when you begin distribution of Opaque copies in quantity, to ensure
that this Transparent copy will remain thus accessible at the stated
location until at least one year after the last time you distribute an
Opaque copy (directly or through your agents or retailers) of that
edition to the public.

It is requested, but not required, that you contact the authors of the
Document well before redistributing any large number of copies, to give
them a chance to provide you with an updated version of the Document.


\section{MODIFICATIONS}
\label{modifications}

You may copy and distribute a Modified Version of the Document under
the conditions of sections~\ref{verbatim} and \ref{copying} above,
provided that you release
the Modified Version under precisely this License, with the Modified
Version filling the role of the Document, thus licensing distribution
and modification of the Modified Version to whoever possesses a copy
of it.  In addition, you must do these things in the Modified Version:

\renewcommand{\labelenumi}{\Alph{enumi}.}
\begin{enumerate}
\item Use in the Title Page (and on the covers, if any) a title distinct
   from that of the Document, and from those of previous versions
   (which should, if there were any, be listed in the History section
   of the Document).  You may use the same title as a previous version
   if the original publisher of that version gives permission.
\item List on the Title Page, as authors, one or more persons or entities
   responsible for authorship of the modifications in the Modified
   Version, together with at least five of the principal authors of the
   Document (all of its principal authors, if it has fewer than five),
   unless they release you from this requirement.
\item State on the Title page the name of the publisher of the
   Modified Version, as the publisher.
\item Preserve all the copyright notices of the Document.
\item Add an appropriate copyright notice for your modifications
   adjacent to the other copyright notices.
\item Include, immediately after the copyright notices, a license notice
   giving the public permission to use the Modified Version under the
   terms of this License, in the form shown in the Addendum below.
\item Preserve in that license notice the full lists of Invariant Sections
   and required Cover Texts given in the Document's license notice.
\item Include an unaltered copy of this License.
\item Preserve the section Entitled ``History'', Preserve its Title, and add
   to it an item stating at least the title, year, new authors, and
   publisher of the Modified Version as given on the Title Page.  If
   there is no section Entitled ``History'' in the Document, create one
   stating the title, year, authors, and publisher of the Document as
   given on its Title Page, then add an item describing the Modified
   Version as stated in the previous sentence.
\item Preserve the network location, if any, given in the Document for
   public access to a Transparent copy of the Document, and likewise
   the network locations given in the Document for previous versions
   it was based on.  These may be placed in the ``History'' section.
   You may omit a network location for a work that was published at
   least four years before the Document itself, or if the original
   publisher of the version it refers to gives permission.
\item For any section Entitled ``Acknowledgements'' or ``Dedications'',
   Preserve the Title of the section, and preserve in the section all
   the substance and tone of each of the contributor acknowledgements
   and/or dedications given therein.
\item Preserve all the Invariant Sections of the Document,
   unaltered in their text and in their titles.  Section numbers
   or the equivalent are not considered part of the section titles.
\item Delete any section Entitled ``Endorsements''.  Such a section
   may not be included in the Modified Version.
\item Do not retitle any existing section to be Entitled ``Endorsements''
   or to conflict in title with any Invariant Section.
\item Preserve any Warranty Disclaimers.

\end{enumerate}

If the Modified Version includes new front-matter sections or
appendices that qualify as Secondary Sections and contain no material
copied from the Document, you may at your option designate some or all
of these sections as invariant.  To do this, add their titles to the
list of Invariant Sections in the Modified Version's license notice.
These titles must be distinct from any other section titles.

You may add a section Entitled ``Endorsements'', provided it contains
nothing but endorsements of your Modified Version by various
parties--for example, statements of peer review or that the text has
been approved by an organization as the authoritative definition of a
standard.

You may add a passage of up to five words as a Front-Cover Text, and a
passage of up to 25 words as a Back-Cover Text, to the end of the list
of Cover Texts in the Modified Version.  Only one passage of
Front-Cover Text and one of Back-Cover Text may be added by (or
through arrangements made by) any one entity.  If the Document already
includes a cover text for the same cover, previously added by you or
by arrangement made by the same entity you are acting on behalf of,
you may not add another; but you may replace the old one, on explicit
permission from the previous publisher that added the old one.

The author(s) and publisher(s) of the Document do not by this License
give permission to use their names for publicity for or to assert or
imply endorsement of any Modified Version.


\section{COMBINING DOCUMENTS}
\label{combining}

You may combine the Document with other documents released under this
License, under the terms defined in section~\ref{modifications}
above for modified
versions, provided that you include in the combination all of the
Invariant Sections of all of the original documents, unmodified, and
list them all as Invariant Sections of your combined work in its
license notice, and that you preserve all their Warranty Disclaimers.

The combined work need only contain one copy of this License, and
multiple identical Invariant Sections may be replaced with a single
copy.  If there are multiple Invariant Sections with the same name but
different contents, make the title of each such section unique by
adding at the end of it, in parentheses, the name of the original
author or publisher of that section if known, or else a unique number.
Make the same adjustment to the section titles in the list of
Invariant Sections in the license notice of the combined work.

In the combination, you must combine any sections Entitled ``History''
in the various original documents, forming one section Entitled
``History''; likewise combine any sections Entitled ``Acknowledgements'',
and any sections Entitled ``Dedications''.  You must delete all sections
Entitled ``Endorsements''.


\section{COLLECTIONS OF DOCUMENTS}
\label{collections}

You may make a collection consisting of the Document and other documents
released under this License, and replace the individual copies of this
License in the various documents with a single copy that is included in
the collection, provided that you follow the rules of this License for
verbatim copying of each of the documents in all other respects.

You may extract a single document from such a collection, and distribute
it individually under this License, provided you insert a copy of this
License into the extracted document, and follow this License in all
other respects regarding verbatim copying of that document.


\section{AGGREGATION WITH INDEPENDENT WORKS}
\label{aggregation}

A compilation of the Document or its derivatives with other separate
and independent documents or works, in or on a volume of a storage or
distribution medium, is called an ``aggregate'' if the copyright
resulting from the compilation is not used to limit the legal rights
of the compilation's users beyond what the individual works permit.
When the Document is included in an aggregate, this License does not
apply to the other works in the aggregate which are not themselves
derivative works of the Document.

If the Cover Text requirement of section~\ref{copying} is applicable to
these copies of the Document, then if the Document is less than one half
of the entire aggregate, the Document's Cover Texts may be placed on
covers that bracket the Document within the aggregate, or the
electronic equivalent of covers if the Document is in electronic form.
Otherwise they must appear on printed covers that bracket the whole
aggregate.


\section{TRANSLATION}
\label{translation}

Translation is considered a kind of modification, so you may
distribute translations of the Document under the terms of
section~\ref{modifications}.
Replacing Invariant Sections with translations requires special
permission from their copyright holders, but you may include
translations of some or all Invariant Sections in addition to the
original versions of these Invariant Sections.  You may include a
translation of this License, and all the license notices in the
Document, and any Warranty Disclaimers, provided that you also include
the original English version of this License and the original versions
of those notices and disclaimers.  In case of a disagreement between
the translation and the original version of this License or a notice
or disclaimer, the original version will prevail.

If a section in the Document is Entitled ``Acknowledgements'',
``Dedications'', or ``History'', the requirement
(section~\ref{modifications}) to Preserve
its Title (section~\ref{applicability}) will typically require
changing the actual title.


\section{TERMINATION}
\label{termination}

You may not copy, modify, sublicense, or distribute the Document except
as expressly provided for under this License.  Any other attempt to
copy, modify, sublicense or distribute the Document is void, and will
automatically terminate your rights under this License.  However,
parties who have received copies, or rights, from you under this
License will not have their licenses terminated so long as such
parties remain in full compliance.


\section{FUTURE REVISIONS OF THIS LICENSE}
\label{future}

The Free Software Foundation may publish new, revised versions
of the GNU Free Documentation License from time to time.  Such new
versions will be similar in spirit to the present version, but may
differ in detail to address new problems or concerns.  See
http://www.gnu.org/copyleft/.

Each version of the License is given a distinguishing version number.
If the Document specifies that a particular numbered version of this
License ``or any later version'' applies to it, you have the option of
following the terms and conditions either of that specified version or
of any later version that has been published (not as a draft) by the
Free Software Foundation.  If the Document does not specify a version
number of this License, you may choose any version ever published (not
as a draft) by the Free Software Foundation.


\section*{ADDENDUM: How to use this License for your documents}

To use this License in a document you have written, include a copy of
the License in the document and put the following copyright and
license notices just after the title page:

\begin{quote}
    Copyright \copyright\ YEAR  YOUR NAME.
    Permission is granted to copy, distribute and/or modify this document
    under the terms of the GNU Free Documentation License, Version 1.2
    or any later version published by the Free Software Foundation;
    with no Invariant Sections, no Front-Cover Texts, and no Back-Cover Texts.
    A copy of the license is included in the section entitled ``GNU
    Free Documentation License''.
\end{quote}

If you have Invariant Sections, Front-Cover Texts and Back-Cover Texts,
replace the ``with...Texts.'' line with this:

    with the Invariant Sections being LIST THEIR TITLES, with the
    Front-Cover Texts being LIST, and with the Back-Cover Texts being LIST.

If you have Invariant Sections without Cover Texts, or some other
combination of the three, merge those two alternatives to suit the
situation.

If your document contains nontrivial examples of program code, we
recommend releasing these examples in parallel under your choice of
free software license, such as the GNU General Public License,
to permit their use in free software.


==> hyperref/hyperref.tex <==
\foilhead{Bookmarks with package *hyperref*}
\begin{itemize}
\item Places for options.
\item Options for bookmarks.
\item Creating bookmarks.
\item Replacement methods.
\end{itemize}

\begingroup
\hypersetup{bookmarksopenlevel=2}

\subfoilhead{Places for \texorpdfstring{*hyperref* }{}options}
\begin{enumerate}
\item Global: \Blue{\cms{documentclass}}\Code{[}\dots\Code{]} (*eg* driver)
\item Package: \Blue{\cms{usepackage}}\Code{[}\dots\Code{]}
\item Configuration file: \Blue{\File{hyperref.cfg}} with \cms{hypersetup}
\item After package has been loaded:
  \Blue{\cms{hypersetup}}\Code{\{}\dots\Code{\}}\\
  (*eg* *pdf* information options)
\end{enumerate}


\subfoilhead[-1.5\baselineskip]{Bookmark options}

\begingroup
  \def\sep{0.5ex}
  \noindent
  \Red{\Option{bookmarks}}: Make bookmarks
    (default: \Green{\Value{true}}).\\[\sep]
  \Red{\Option{bookmarksnumbered}}: Put section numbers in bookmarks
    (\Green{\Value{false}}).\\[\sep]
  \Red{\Option{bookmarksopen}}: Open up bookmark tree
     (default: \Green{\Value{false}}).\\[\sep]
  \Red{\Option{bookmarksopenlevel}}: Level, to which bookmarks are
     open.\\[\sep]
  \Red{\Option{pdfpagemode}}: How document starts when opened
     (default: \Green{\Value{None}}):
  \begingroup
    \mbox\qquad\Blue{\Option{None}}: Neither outlines nor thumbnails are visible.\\
    \mbox\qquad\Blue{\Option{UseOutlines}}, \Blue{\Option{UseThumbs}}:
      Outlines, thumbnails are visible.\\
    \mbox\qquad\Blue{\Option{FullScreen}}: Full-screen mode.\\[\sep]
  \endgroup
  \Red{\Option{unicode}}: Bookmarks in *unicode*
     (\Green{\Value{false}}). After package has been\\
     \mbox\qquad loaded, it switches between *unicode* and *pdfdocencoding*.
\endgroup


\subfoilhead[-0.5\baselineskip]{%
  \texorpdfstring{Bookmarks by \abbr{sectioning}}{\abbr{Sectioning}} %
  commands
}
\label{sec:bmbysec}

\begin{itemize}
\item Automatically addition of bookmarks by:
      \begin{itemize}
      \item \cms{part}, \cms{chapter}, \cms{section}, \cms{subsection}, \dots
      \item \cms{addcontentsline}
      \end{itemize}
\item Help file \Blue{\Code{\textsl{\cms{jobname}}.out}}:
      \begin{itemize}
      \item It is written in the \Green{first} run.
      \item The bookmarks are set in the \Green{second} run.
      \item There is \Green{\emph{no}} ``rerun'' warning.
      \end{itemize}
\end{itemize}


\subfoilhead{Tree structure\texorpdfstring{ of bookmarks}{}}

\begin{itemize}
\item Subentries must be added to \Blue{direct} ancestores,
      \Blue{not} grandparents.
\item If an intermediate level is omitted, the leaf starts \Blue{leftmost}:
      \begin{quote}
        \def\sub{\Red{\ensuremath{\rightarrow}}}%
        \def\ver{\Red{\ensuremath{\|}}}%
        \begin{tabular}{@{}lll@{}}
        &\Blue{table of contents}&\Blue{bookmarks}\\
        \hline
        \cms{part}\Code{\{I\}}&\ver{Part I}&\ver{main entry}\\
        \cms{chapter}\Code{\{5\}}&%
          \ver\sub{Chapter I.5}&\ver\sub{subentry}\\
        \cms{subsection}\Code{\{1\}}&
          \ver\sub\sub\sub{Subsection I.5.0.1}&\ver{main entry}\\
        \end{tabular}
      \end{quote}
\end{itemize}


\subfoilhead[-\baselineskip]{\texorpdfstring{Creating bookmarks with }{}\cms{pdfbookmark}}

\begin{itemize}
\item The bookmarks of *sectioning* commands have an \Red{level} number:
      \par\noindent
      \begin{tabular}{@{}lc@{ }c@{ }c@{ }c@{ }c@{}}
      documentclass&\cms{part}&\cms{chapter}&%
        \cms{section}&\cms{subsection}&\dots\\
      \Class{book}/\Class{report}:&\Red{\llap{$-$}1}&%
        \Red0&\Red1&\Red2&\dots\\
      \Class{article}:&\Red0&&\Red1&\Red2&\dots\\
      \end{tabular}
\item Syntax of \Blue{\cms{pdfbookmark}} (default for level: \Red{0}):
      \begin{quote}
        \Blue{\cms{pdfbookmark}}%
          \Code{[\Red{\emph{level}}]\{\emph{bookmark text}\}%
            \{\Green{\emph{anchor name}}\}}
      \end{quote}
\item \Blue{\cms{currentpdfbookmark}}%
        \Code{\{\emph{bookmark}\}\{\Green{\emph{anchor}}\}}%
        \commentchar\ \Red{current level}
\item \Blue{\cms{subpdfbookmark}}%
        \Code{\{\emph{bookmark}\}\{\Green{\emph{anchor}}\}}%
        \commentchar\ \Red{current level + 1}
\end{itemize}


\subsubfoilhead[-\baselineskip]{Using anchors%
  \texorpdfstring{ with \cms{pdfbookmark}}{}%
}

\begin{itemize}
\item An \Green{anchor name} consists of the argument and
      the level:
      \begin{quote}
        \Blue{\cms{pdfbookmark}}\Code{[\Red0]\{Titlepage\}\{\Green{tit}\}}%
          \Code{\commentchar\ }anchor: \Code{\Green{tit}.\Red0}
      \end{quote}
\item The bookmark can point to another \Green{target} (\Green{anchor}):
      \begin{quote}\small
        \cms{hypertarget}\Code{\{\Green{place.}\Red{1}\}\{\}}
      \end{quote}
      Redirecting the bookmark to the previous defined \Green{target}:
      \begin{quote}\small
        \cms{begingroup}\\
        *ind*\cms{makeatletter}\\
        *ind*\cms{def}\cms{hyper@anchorstart}\Code{ \#1}%
          \cms{hyper@anchorend}\Code{\{\}\%}\\
        *ind*\Blue{\cms{pdfbookmark}}\Code{[\Red1]\{Go to the place\}\{\Green{place}\}\%}\\
        \cms{endgroup}
      \end{quote}
\end{itemize}

\endgroup
\endinput


==> hyperref/links.tex <==
\subfoilhead[-\baselineskip]{Links}

\begin{Nav}{\NavBookmarks\NavQuit}

\begin{smallpar}
\let\Blue\empty
\pdfadjustspacing=1
\noindent
\begingroup
\def\it{\textbullet}%
\def\sep{1ex}%
\begin{tabularx}{\linewidth}{@{}l@{ }X@{}}
  \it&\Blue{*pdfspec*} (version 1.3):\newline
    \link{http://partners.adobe.com/asn/developer/PDFS/TN/PDFSPEC.PDF}%
    \tabularnewline[\sep]
  \it&\Blue{*pdftex*}:
    \begingroup
      \settoheight{\dimen0}{\mbox{\^e}}%
      \settoheight{\dimen1}{\mbox{e}}%
      \addtolength{\dimen0}{-\dimen1}%
    (H\`an Th\rlap{\raise\dimen0\hbox{\'{}}}\^e Th\`anh):
    \endgroup
    \newline
    \link{http://www.tug.org/applications/pdftex/}\newline
    Win32: \link{ftp://ftp.ese-metz.fr/pub/TeX/win32-beta/}%
    \tabularnewline[\sep]
  \it&\Blue{*hyperref*} (Sebastian Rahtz):\hfill
    \link{ftp://ctan.tug.org/tex-archive/macros/latex/contrib/supported/hyperref/}%
    \newline
    Test versions:\newline
    \link{http://www.tug.org/applications/hyperref/hyperref.zip}
    \tabularnewline[\sep]
  \it&\Blue{*hypbmsec*} (Heiko Oberdiek):\hfill
    \link{ftp://ctan.tug.org/tex-archive/macros/latex/contrib/supported/oberdiek/}%
    \tabularnewline[\sep]
  \it&\Blue{*thumbpdf*} (Heiko Oberdiek):\newline
    \link{ftp://ctan.tug.org/tex-archive/macros/pdftex/thumbpdf/}%
\end{tabularx}
\endgroup
\end{smallpar}

%\SetNav{\NavFull\NavSep\NavPrev\NavSep\NavQuit}
\end{Nav}

\endinput


==> hyperref/navbook.tex <==
\newcommand{\bmaction}[3][0]{%
  \begingroup
    \pdfstringdef\x{#3}%
    \pdfoutline user {<</S /Named /N /#2>>} count #1 {\x}%
  \endgroup
}
\bmaction[-3]{NOP}{Navigation}
  \bmaction[2]{FullScreen}{Full-screen}
    \bmaction{PageOnly}{Page only}
    \bmaction{ShowThumbs}{Thumbnails}
  \bmaction[6]{NOP}{Selecting pages}
    \bmaction{PrevPage}{Previous page}
    \bmaction{NextPage}{Next page}
    \bmaction{GoBack}{Go back}
    \bmaction{GoForward}{Go forward}
    \bmaction{FirstPage}{First page}
    \bmaction{LastPage}{Last page}
  \bmaction[2]{GeneralInfo}{General document information}
    \bmaction{ShowHideMenuBar}{Menu bar}
    \bmaction{ShowHideToolBar}{Tool bar}

\endinput


==> hyperref/pdfextra.tex <==
\foilhead{Additional features of \abbr{pdf} format}
\noindent
Hyperref does not support all possibilities of *pdf* format, e.\,g.:
\begin{itemize}
  \let\Blue\empty
  \item \Blue{\Code{/CreationDate}} and \Blue{\Code{/ModDate}}.
  \item \Blue{Bookmarks} with \Blue{other functions}.
\end{itemize}
The following examples uses commands of \empty{*pdftex*}.

\subfoilhead{Bookmarks with other functions}
\begin{Nav}{\NavBookmarks\NavPage}

\begin{itemize}
  \item Menu functions of AcrobatReader, sound, video, \dots
  \item *pdftex* low level command:\\[1ex]
        \code[red]<\pdfoutline>\ \emph{\code<action>}\
        \code<count>\ \emph{\code[blue]<n>}\
        \code<{>\emph{\code<text>}\code<}>
        \begin{itemize}
          \item
            The absolute value of \emph{\code[blue]<n>}\ is the
            count of the direct subentries.
          \item
            If \emph{\code[blue]<n>}\ is negative, the
            subentries are closed.
        \end{itemize}
\end{itemize}


\subfoilhead{Link to external file}
\noindent
The *pdfspec* contains the possible actions on page 96.\\
At last a bookmark that points to that page:
\begingroup
  \edef\({\string(}
  \edef\){\string)}
\begin{verbatim}
$Blue(\pdfoutline)
  user {<<$Green(/S /GoToR /F $(pdfspec.pdf$) /D [95 /Fit])>>}
  count 0 {$empty(Description of actions)}
\end{verbatim}
\endgroup

\end{Nav}

\endinput


==> hyperref/pdfinfo.tex <==
\hypersetup!{%
  pdftitle!    = {PDF information and navigation elements},
  pdfsubject!  = {Slides for talk at EuroTeX'99 in Heidelberg},
  pdfkeywords! = {pdf, hyperref, bookmarks, thumbnails},
  pdfauthor!   = {\textcopyright\ Heiko Oberdiek},
  pdfcreator!  = {\LaTeX\ with package \flqq hyperref\frqq},
  pdfproducer! = {pdfeTeX-0.\the\pdftexversion\pdftexrevision},
}
\pdfinfo!{/CreationDate! (D:19990909000000-01'00')}

==> hyperref/psd.tex <==

\foilhead[-\baselineskip]{\cms{pdfstringdef}%
  \texorpdfstring{  converts \abbr{tex} to \abbr{pdf} strings}{}}

\noindent
Syntax: \Blue{\cms{pdfstringdef}}\Code{\{\emph{\cms{command}}\}%
    \{\emph{*tex* string}\}}

\begin{enumerate}
\item Selecting the encoding *PD1* or *PU*.
\item Redefinitions of many commands, so that they
      produce correct\\
      results or do not harm.
\item Expansion of the string.
\item Token checks and removal of forbidden tokens with 
      comprehensive\\ 
      warnings.
\end{enumerate}


\subfoilhead[-.5\baselineskip]{Redefinitions%
  \texorpdfstring{ by \cms{pdfstringdef}}{}}
\begin{itemize}
\item Redefinitions to get correct results, *eg*:
      \begin{itemize} 
      \item Glyph commands: \cms{\{}, \cms{\%}, \cms{space}, \cms{dots},
            \dots
      \item Logos: \cms{TeX}, \cms{LaTeX}, \cms{MF}, \dots
      \end{itemize}
\item Many tokens are removed silently, *eg*:
      \begin{itemize}
      \item *latex* commands: \cms{label}, \cms{index}, 
           \cms{textbf}, \dots
      \item Stomach tokens: curly group braces, \cms{relax} (\cms{protect}), 
            \dots
      \end{itemize}
\item The behaviour of \cms{xspace} is simulated.
\end{itemize}

\endinput


==> hyperref/replace.tex <==
\foilhead{Replacement methods}

\begin{itemize}
%\item \code[blue]<\texorpdfstring>\ provides an alternative.
\item \Blue{\cms{texorpdfstring}} choices one of its arguments:\\
      a *tex* or a *pdf* string.
\item \code[blue]<\pdfstringdefPreHook>\ is a place for redefining commands.\\
      Additions are made by \code[blue]<\pdfstringdefDisableCommands>.
\item Package \Blue{*hypbmsec*} extends the \code<\section>\ commands.
\end{itemize}


\subfoilhead{\cms{texorpdfstring} method}
\noindent
Syntax: \Red{\cms{texorpdfstring}}%
        \Green{\Code{\{*tex* string\}}}%
        \Blue{\Code{\{*pdf* string\}}}

\noindent
Example:

\noindent
  \cms{section}\Code{\{}\Red{\cms{texorpdfstring}}%
  %\Code{\emph{\%}}%
  \Green{\Code{\{H\$\_2\$O\}}}%
  %\Code{\emph{\%}}%
  \Blue{\Code{\{Water\}}}%
  %\Code{\emph{\%}}%
  \Code{\}}


\subfoilhead[-1\baselineskip]{Hook for private macro redefinitions}

\begin{itemize}
\item \Red{\cms{pdfstringdefPreHook}} is called, before expanding the string.
\item \Red{\cms{pdfstringdefDisableCommands}} adds user redefinitions to\\
      \cms{pdfstringdefPreHook}

  \Blue{\cms{pdfstringdefDisableCommands}}\Code{\{\commentchar}\\
  *ind*\cms{renewcommand}\Code{\{\cms{textcolor}\}[1]\{\#1\}\commentchar}\\
  *ind*\cms{renewcommand}\Code{\{\cms{url}\}}\Code{\{}\empty{\cms{pdfstringdefwarn}}%
    \Code{\{\cms{url}\}}\Code{\}\commentchar}\\
  *ind*\cms{let}\cms{textcolor}\cms{@gobble}\\
  \Code{\}}
\item \Red{\cms{pdfstringdefwarn}} prints a warning message.
\end{itemize}


\subfoilhead[-\baselineskip]{Package \Package{hypbmsec}}

\begin{itemize}
\item The syntax of \cms{section} commands is extended:
      \begin{itemize}
      \item Second optional bookmark argument.
      \item Bookmark in parentheses.
      \end{itemize}
\item Syntax:
  \def\txt{\Blue{\textsl{text}}}%
  \def\toc{\Green{\textsl{toc/head}}}%
  \def\out{\Red{\textsl{bookmark}}}%
  \settowidth{\dimen0}{\toc}%
  \settowidth{\dimen1}{\out}%
  \addtolength{\dimen1}{-\dimen0}%
  \setlength{\dimen1}{.5\dimen1}%
  \edef\toc{\noexpand\Green{\noexpand\textsl{toc%
    \noexpand\hspace{\the\dimen1}/\noexpand\hspace{\the\dimen1}head}}}%
  \settowidth{\dimen0}{\textbf{]\{}}%
  \settowidth{\dimen1}{ = }%
  \addtolength{\dimen0}{-\dimen1}%
  \setlength{\dimen0}{-.5\dimen0}%
  \edef\xsp{\noexpand\hspace{\the\dimen0}}%
  \def\({\textbf{(}\,}%
  \def\){\,\textbf{)}}%
  \def\[{\textbf{[}\,}%
  \def\]{\,\textbf{]}}%
  \def\{{\textbf{\orgbraceleft}\,}%
  \def\}{\,\textbf{\orgbraceright}}%
  \def\section{\cms{section}}%
  \def~{ = }%
  \begin{tabular}[t]{@{}l@{ }c@{}c@{}c@{}c@{}c@{}l@{}}
    \section&\{&\toc&~&\out&~&\txt\}\\
    \section&\[&\toc&~&\out&\]\,\{&\txt\}\\[1ex]
    \section&\[&\toc&\]\,\[&\out&\]\,\{&\txt\}\\[1ex]
    \section&\(&\out&\)\,\{&\toc&~&\txt\}\\
    \section&\[&\toc&\]\,\(&\out&\)\,\{&\txt\}\\
    \section&\(&\out&\)\,\[&\toc&\]\,\{&\txt\}\\
  \end{tabular}
\end{itemize}


\endinput

The next version of package *hypbmsec* will know the
option \Blue{\Option{startotoc}}:
The starred *sectioning* commands are included in the table
of contents and in the outline tree automatically.
For options \Blue{\Option{infix}} and \Blue{\Option{prefix}}
see \secref{sec:addcontentsline}.

\endinput


==> hyperref/strings.tex <==
\clearpage
\pdfbookmark[0]{Strings}{string}

\begingroup
\hypersetup{bookmarksopenlevel=2}

\subfoilhead[-\baselineskip]{\abbr{pdf} strings}

\begin{itemize}
\item Examples, where *pdf* strings are used:
      \begin{quote}
      Bookmark names, information dictionaries, text annotations
      \end{quote}
\item *pdf* strings follow the *postscript* rules:
      \begin{itemize}
      \item Delimited by parentheses: \Code{\Blue{(}This is a string\Blue{)}}
      \item Escape sequences for white space, \Blue{\cms{(}}, \Blue{\cms{)}},
            \Blue{\cms{}\cms{}};\\
            octal notation, *eg*: `\"a\"o\"u\ss' = 
            \Code{(}\Blue{\cms{344}\cms{366}\cms{374}\cms{337}}\Code{)}
      \end{itemize}
\item 
%      $\vcenter{\mbox{%
        \begin{tabular}[t]{@{}l@{ }l@{}}
          \Blue{*pdfdocencoding*}:&8bit, superset of *isolatin1*\\
          \Blue{*unicode*}:&16bit, *acroread* version $\ge$ 4\\
        \end{tabular}%
%      }}$ 
\end{itemize}


\clearpage
\pdfbookmark[1]{\abbr{tex} strings}{strings}

\subsubfoilhead[-.5\baselineskip]{Digestion of \abbr{tex}}

\begingroup
\newenvironment{organ}[2]{%
  \begin{minipage}[t]{\linewidth}%
    \vspace{#2}%
    \begin{tabbing}%
      \begin{tabular}{@{\textbullet\ }l@{}}
        \multicolumn{1}{@{}l@{}}{%
%          \phantom{\textbullet\ }%
          \textbf{\large\Blue{#1}}}\\[0.5ex]
}{
      \end{tabular}%
    \end{tabbing}%
  \end{minipage}%
}

\makeatletter
\let\fbox\@firstofone

\noindent
\fbox{%
\begin{organ}{Eyes}{0pt}
  Reading input lines\\
  Catcodes are set
\end{organ}}%
\hfill
\fbox{%
\begin{organ}{Mouth}{2\baselineskip}
  Forming tokens\\
  Expansion of macros
\end{organ}}%
\hfill
\fbox{%
\begin{organ}{Stomach}{4\baselineskip}
  Assignments\\
  Typesetting
\end{organ}}%

\endgroup


\subsubfoilhead[-.5\baselineskip]{Differences between mouth and stomach}

\noindent
\begin{tabular}{@{}lll@{}}
  &\Blue{\textbf{mouth}}&
   \Blue{\textbf{stomach}}\\[1ex]
``zero'':& \code<\empty>&\code<\relax>\\[0.5ex]
\code<{...}>:&parameter&group\\[0.5ex]
variable:&read and check&assignments\\[0.5ex]
fonts:&--&different fonts and encodings\\
&&ligatures\\[0.5ex]
Commands:&\code<\string>, \code<\number>&\code<\def>, \code<\hbox>, \code<$>\\
&\code<\if>, \code<\the>&\code<\begingroup>, \code<\special>
\end{tabular}


\subfoilhead[-.5\baselineskip]{\abbr{tex} into \abbr{pdf} strings}

\begin{itemize}
\item Reusing the argument of *sectioning* commands (*tex* string)\\
      for the bookmarks (*pdf* strings).
\item Limitations because of missing stomach digestion:
      \begin{itemize}
      \item No manipulation of boxes, no mathematics, no colors, \dots
      \item No change of fonts or encodings, no ligatures.
      \item No assignments (\cms{xspace} uses \cms{futurelet}).
      \item Unexpandable commands appear verbatim.
      \end{itemize}
\end{itemize}


\endgroup
\endinput

==> hyperref/summary.tex <==
\clearpage
\pdfbookmark[0]{End}{ende}

\subfoilhead[-1.5\baselineskip]{Summary}
\begin{itemize}
  \item \Red{General document information}:
    \begin{itemize}
      \item Options in \code[blue]<\hypersetup>\
            after \cms{usepackage}\Code{\{hyperref\}}.
    \end{itemize}
  \item \Red{Bookmarks}:
    \begin{itemize}
      \item Automatically added by \Blue{*hyperref*}.
      \item \Blue{Oral expansion}, no stomach commands (exceptions).
      \item Replacement methods: \code[blue]<\texorpdfstring>,\\
            \code[blue]<\pdfstringdefDisableCommands>, and
            \Blue{*hypbmsec*}.
      \item Low level commands only for special effects.
    \end{itemize}
  \item \Red{Thumbnails}: Automatically added by \Blue{*thumbpdf*}.
\end{itemize}


==> hyperref/thumb.tex <==

\foilhead{Thumbnails}
\begin{Nav}{\NavThumbnails\NavBookmarks}
\thisthumb{zurueck}
\begin{itemize}
  \item Another method for navigation:
    \begin{itemize}
      \item Choosing pages.
      \item Selecting page areas.
    \end{itemize}
  \item Contents:
    \begin{itemize}
      \item Thumbnail sketches of the pages.
      \item Other pictograms, symbols, \dots
      \item Empty.
    \end{itemize}
\end{itemize}


\subfoilhead{Adding thumbnails with \abbr{thumbpdf}}
\thisthumb{weiter}
\begingroup
  \centering
  \setlength{\unitlength}{1pt}
  % ca. max: 240mm x 100mm
  % ca. max: 700pt x 300pt
  \def\FileBox#1{\framebox(180,40){\Code{\vphantom{Hg}#1}}}
  \def\ProgBox[#1]#2{\makebox(160,60)[#1]{\vphantom{Hg}#2}}
  \def\Nummer[#1]#2{\makebox(20,60)[#1]{%
    \vphantom{Hg}%
    $\smash{%
      \textsf{\textcircled{\vphantom{\large#2}\Blue{\small#2}}}%
    }$%
  }}
  \def\Down{\makebox(0,0)[b]{\DOWNarrow}}%
  \def\Up{\makebox(0,0)[t]{\UParrow}}%
  \def\Right{\makebox(0,0)[r]{\RIGHTarrow}}%
  \begin{picture}(670,250)
    % Dateinamen
    \put(80,0){\FileBox{thumbdta.tex}}
    \put(80,100){\FileBox{\emph{jobname}.pdf}}
    \put(80,200){\FileBox{\emph{jobname}.tex}}
    \put(470,200){\FileBox{\Red{\emph{jobname}.pdf}}}
    % Pfeile
    \put(170,200){\line(0,-1){60}}
    \put(170,140){\Down}
    \put(170,100){\line(0,-1){60}}
    \put(170,40){\Down}
    \put(260,220){\line(1,0){210}}
    \put(470,220){\Right}
    \put(260,20){\line(1,0){105}}
    \put(365,20){\line(0,1){160}}
    \put(365,180){\Up}
    % Nummern
    \put(190,140){\Nummer[l]{1}}
    \put(190,40){\Nummer[l]{2}}
    \put(280,230){\Nummer[lb]{3}}
    % Programme
    \put(-10,40){\ProgBox[r]{*thumbpdf*}}
    \put(-10,140){\ProgBox[r]{*pdftex*}}
    \put(285,230){\ProgBox[b]{*pdftex*}}
    \put(285,150){\ProgBox[t]{\Code{thumbpdf.sty}}}
  \end{picture}
\endgroup

\subfoilhead[-\baselineskip]{How \abbr{thumbpdf} works}
\begingroup
  \centering
  \setlength{\unitlength}{1pt}
  % ca. max: 240mm x 100mm
  % ca. max: 700pt x 300pt
  \def\FileBox#1{\framebox(180,40){\Code{\vphantom{Hg}#1}}}
  \def\ProgBox[#1]#2{\makebox(160,60)[#1]{\vphantom{Hg}#2}}
  \def\Down{\makebox(0,0)[b]{\DOWNarrow}}%
  \def\Up{\makebox(0,0)[t]{\UParrow}}%
  \def\Right{\makebox(0,0)[r]{\RIGHTarrow}}%
  \def\Left{\makebox(0,0)[l]{\LEFTarrow}}%
  \begin{picture}(650,340)
    % Dateinamen
    \put(80,0){\FileBox{\Red{thumbdta.tex}}}
    \put(80,100){\FileBox{thumbdta.pdf}}
    \put(80,200){\FileBox{thumb\emph{???}.png}}
    \put(80,300){\FileBox{\emph{jobname}.pdf}}
    \put(420,150){\FileBox{thumbopt.tex}}
    \put(420,240){\FileBox{\emph{other images}}}
    % Pfeile
    \put(170,300){\line(0,-1){60}}
    \put(170,240){\Down}
    \put(170,200){\line(0,-1){60}}
    \put(170,140){\Down}
    \put(170,100){\line(0,-1){60}}
    \put(170,40){\Down}
    \put(360,170){\line(1,0){60}}
    \put(360,170){\Left}
    \put(510,240){\line(0,-1){50}}
    \put(510,190){\Down}
    % Programme
    \put(-10,40){\ProgBox[r]{\textsf{perl}}}
    \put(-10,140){\ProgBox[r]{*pdftex*}}
    \put(190,140){\ProgBox[l]{\Code{thumbpdf.tex}}}
    \put(-10,240){\ProgBox[r]{*gs*}}
  \end{picture}
\endgroup


\iffalse %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subfoilhead{Thumbnails and *pdftex*}
\begin{itemize}
\item There is no direct support.
\item \code[blue]<\pdfimage> (*pdftex* versions below 0.14):
  \begin{itemize}
    \item[$+$] Image works as thumbnail.
    \item[$-$] No access to the image object number.
    \item[$-$] Image is on the page, must be
               moved out of the page.
  \end{itemize}
\item Low level commands
  \code[blue]<\pdfobj>\ and \code[blue]<\pdflastobj>\ are possible.
\end{itemize}

\clearpage
\pdfbookmark[1]{Project *thumbpdf*}{thumbpdf}
\subsubfoilhead[-\baselineskip]{Solution\texorpdfstring{ of project *thumbpdf*}{}}

\begin{enumerate}
  \item Generating the thumbnails \Blue{\file{thumb???.png}} by \Red{*gs*}.
  \item \Red{*pdftex*} runs \Red{\file{thumbpdf.tex}},
        thumbnails included by \code[blue]<\pdfimage>.
  \item The perl script \Red{\file{thumbpdf.pl}} reads
        \Blue{\file{thumbpdf.pdf}} and writes\\
        the object data in a *tex*
        readable form \Blue{\file{thumbdta.tex}}.
  \item Package \Red{\file{thumbpdf.sty}} inputs \Blue{\file{thumbdta.tex}},
        that contains the\\
        thumbnails as *pdf* objects (\code[blue]<\pdfobj>).
  \item The object numbers of the thumbnails (\code[blue]<\pdflastobj>)
        are added\\
        to the page attributes (\code[blue]<\pdfpageattr>).
\end{enumerate}


\subsubfoilhead[-.5\baselineskip]{User interface\texorpdfstring{ of *thumbpdf*}{}}

\begin{itemize}
  \def\master{\textsl{master}}%
  \item Command lines (\file{\master.tex} inputs \file{thumbpdf.sty}):
    \begin{enumerate}
      \item \texttt{\Blue{pdf}(\Blue{e},\Blue{la})\Blue{tex \master.tex}}
      \item \Blue{\texttt{thumbpdf \master}}
      \item \texttt{\Blue{pdf}(\Blue{e},\Blue{la})\Blue{tex \master.tex}}
    \end{enumerate}
  \item Another program than *gs* can be used:
    \begin{enumerate}
      \item[2a.] \Blue{\texttt{\textsl{ProgramThatGeneratesThumbnails} \master.pdf}}
      \item[2b.] \Blue{\texttt{thumbpdf}}
    \end{enumerate}
\end{itemize}

\fi %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subfoilhead[-\baselineskip]{Other images as thumbnails}

\begin{itemize}
\item With \Blue{\cms{thumb}} other images are declared as
      thumbnails in the\\ 
      optional file \Blue{\file{thumbopt.tex}}.
\item \Blue{\cms{thisthumb}} sets the thumbnail for the current page.
\end{itemize}
\begingroup
  \let\Red\Green
  \centering
  \begin{tabular}{@{}l@{\quad$\rightarrow$\quad}l@{}}
    \multicolumn{1}{@{}l}{\empty{\File{thumbopt.tex}}}&%
      \File{\emph{jobname}.tex}\\
    \hline
    \empty{\cms{thumb}}\Code{\{\Red{one}\}}&
      \empty{\cms{thisthumb}}\Code{\{\Red{one}\}}\\
    \empty{\cms{thumb}}\Code{\{\Red{one.png}\}}&
      \empty{\cms{thisthumb}}\Code{\{\Red{one.png}\}}\\
    \empty{\cms{thumb}}\Code{[\Red{two}]\{one\}}&
      \empty{\cms{thisthumb}}\Code{\{\Red{two}\}}\\
    \empty{\cms{thumb}}\Code{[\Red{one}]\{./extras/one.png\}}&
      \empty{\cms{thisthumb}}\Code{\{\Red{one}\}}\\
  \end{tabular}
  \par
\endgroup

\end{Nav}

\endinput


==> hyperref/thumbopt.tex <==
\thumb[zurueck]{addthumb/thumb001.png}
\thumb[weiter]{addthumb/thumb002.png}


==> hyperref/title.tex <==
\pdfbookmark[0]{Beginning}{anfang}
\pdfbookmark[1]{Title}{title}

%\date{21st September 1999}% EuroTeX'99
\date{13rd October 1999}% first release for hyperref
\title{*pdf* information and navigation elements with
       hyperref, *pdftex*, and thumbpdf}
\author{Heiko Oberdiek\\\Email{oberdiek@ruf.uni-freiburg.de}}

\begingroup
  \LogoOff\aftergroup\LogoOn
  \Restriction{\unskip\centerline{\NavStart}}%
  \aftergroup\Restriction\aftergroup\empty
  \maketitle
  \begin{abstract}
    \noindent
    Additional possibilities for information and navigation through
    paper-less on-line documents that offer the PDF format.
  \end{abstract}
  \newpage
\endgroup

\subfoilhead{Subjects}
\begin{itemize}
\item General document information\hfill*hyperref*
\item Bookmarks/outlines\hfill*hyperref*
\item Thumbnails\hfill*thumbpdf*
\end{itemize}

\endinput


==> listings/Makefile <==
### Makefile ---
#
# This file generates files required to use the listings package.
#
# $Id$
#
# (c) 2007 Brooks Moses
# (c) 2013-2018 Jobst Hoffmann
#
# This file is distributed under the terms of the LaTeX Project Public
# License from CTAN archives in directory  macros/latex/base/lppl.txt.
# Either version 1.3c or, at your option, any later version.

# remember:
# $<: first element of list of dependees
# $^: list of (all) dependees
# $@: target

# formatting tools
LATEX = pdflatex
MAKEINDEX = makeindex
TEX = tex
# tarring options
ifneq "$(wildcard listings.version)" ""
include listings.version        # version and date of the package
endif
TAR_SRC = $(PACKAGE)-$(VERSION)_source.tgz
EXsvn = --exclude .svn --exclude auto --exclude contrib --exclude requests \
	--exclude support --exclude testing \
	--exclude *.tgz --exclude *.txt

DISTRIBUTION_FILES = ../$(PACKAGE)/$(PACKAGE).pdf \
	../$(PACKAGE)/$(PACKAGE)-devel.pdf \
	../$(PACKAGE)/$(PACKAGE).dtx \
	../$(PACKAGE)/$(PACKAGE).ins \
	../$(PACKAGE)/README \
	../$(PACKAGE)/Makefile \
	../$(PACKAGE)/lstdrvrs.dtx \
	../$(PACKAGE)/lstdrvrs.pdf 
PACKAGE_FILES = $(subst ../$(PACKAGE)/,,$(DISTRIBUTION_FILES))
STY_FILES = listings.cfg listings.sty lstmisc.sty \
	lstlang0.sty lstlang1.sty lstlang2.sty

.SUFFIXES:                              # Delete the default suffixes
.SUFFIXES: .dtx .ins .pdf .sty          # Define our own suffix list

.PHONY: listings pdf pdf-devel tests all

listings: listings.sty

pdf: listings.pdf lstdrvrs.pdf

pdf-devel: listings-devel.pdf

all: listings pdf pdf-devel


listings.sty: listings.ins listings.dtx lstdrvrs.dtx
	$(TEX) $<

listings.pdf: listings.sty
	echo "\PassOptionsToClass{a4paper}{article}" > ltxdoc.cfg
	$(LATEX) ${<:.sty=.dtx}
	$(MAKEINDEX) -s gind.ist ${@:.pdf=}
	$(LATEX) ${<:.sty=.dtx}
	$(LATEX) ${<:.sty=.dtx}
	rm -f ltxdoc.cfg

listings-devel.pdf: listings.sty
	echo "\PassOptionsToClass{a4paper}{article}" > ltxdoc.cfg
	echo "\AtBeginDocument{\AlsoImplementation}" >> ltxdoc.cfg
	$(LATEX) -jobname=${@:.pdf=} ${<:.sty=.dtx}
	$(MAKEINDEX) -s gind.ist ${@:.pdf=}
	$(LATEX) -jobname=${@:.pdf=} ${<:.sty=.dtx}
	$(LATEX) -jobname=${@:.pdf=} ${<:.sty=.dtx}
	rm -f ltxdoc.cfg

lstdrvrs.pdf: lstdrvrs.dtx
	echo "\PassOptionsToClass{a4paper}{article}" > ltxdoc.cfg
	$(LATEX) ${<:.sty=.dtx}
	$(MAKEINDEX) -s gind.ist lstdrvrs
	$(LATEX) ${<:.sty=.dtx}
	$(LATEX) ${<:.sty=.dtx}
	rm -f ltxdoc.cfg

## Testing targets
acm-tests:
	cd testing; make acm

algol-tests:
	cd testing; make algol

bash-tests:
	cd testing; make bash

c++11-tests:
	cd testing; make c++11

cobol-tests:
	cd testing; make cobol

fortran-tests:
	cd testing; make fortran

elisp-tests:
	cd testing; make elisp

gap-tests:
	cd testing; make gap

go-tests:
	cd testing; make go

hansl-tests:
	cd testing; make hansl

llvm-tests:
	cd testing; make llvm

lua-tests:
	cd testing; make lua

mathematica-tests:
	cd testing; make mathematica

python-tests:
	cd testing; make python

scala-tests:
	cd testing; make scala

swift-tests:
	cd testing; make swift

vbscript-tests:
	cd testing; make vbscript

xml-tests:
	cd testing; make xml

tests:
	cd testing; make all

## Clean targets
clean:
	-rm -f  *~ *.aux *.lof *.log *.lot *.tmp *.toc
	-rm -f *.idx *.ind *.glg *.glo *.gls *.ilg *.out
	-rm -f *.bbl *.blg *.brf

clean-results:
	-rm -f *.cfg *.pdf *.prf *.sty

realclean:  clean clean-results

### create packed files
tar-src:
	@$(MAKE) realclean; \
	sed -i -e "s+fileversion{[a-z0-9\.\-]*}+fileversion{$(VERSION)}+g" \
	    -e "s+filedate{[0-9/]*}+filedate{$(DATE)}+g" \
	    -e "s+date{[0-9/]*\\\\enspace+date{$(DATE)\\\\enspace+g" \
	    -e "s+Version [a-z0-9\.\-]*\\\\+Version $(VERSION)\\\\+g" \
		listings.dtx; \
	sed -i -e "s+date{[0-9/]*\\\\enspace+date{$(DATE)\\\\enspace+g" \
	    -e "s+Version [a-z0-9\.\-]*\\\\+Version $(VERSION)\\\\+g" \
	    -e "s+\[[0-9/]* [a-z0-9\.\-]* listings+[$(DATE) $(VERSION) listings+g" \
		lstdrvrs.dtx; \
	cd ..; tar $(EXsvn) -czvf $(PACKAGE)/$(TAR_SRC) $(PACKAGE)

tar-dist: $(PACKAGE_FILES)
	@$(MAKE) realclean; \
	sed -i -e "s+fileversion{[a-z0-9\.\-]*}+fileversion{$(VERSION)}+g" \
	    -e "s+filedate{[0-9/]*}+filedate{$(DATE)}+g" \
	    -e "s+date{[0-9/]*\\\\enspace+date{$(DATE)\\\\enspace+g" \
	    -e "s+Version [a-z0-9\.\-]*\\\\+Version $(VERSION)\\\\+g" \
		listings.dtx; \
	sed -i -e "s+date{[0-9/]*\\\\enspace+date{$(DATE)\\\\enspace+g" \
	    -e "s+Version [a-z0-9\.\-]*\\\\+Version $(VERSION)\\\\+g" \
	    -e "s+\[[0-9/]* [a-z0-9\.\-]* listings+[$(DATE) $(VERSION) listings+g" \
		lstdrvrs.dtx; \
	$(MAKE) listings.pdf; \
	$(MAKE) listings-devel.pdf; \
	$(MAKE) lstdrvrs.pdf; \
	tar cfvz $(PACKAGE)-$(VERSION).tgz $(DISTRIBUTION_FILES);

tagged-release:
	sed -n -e "/Version $(VERSION)/,$$$$w announcement_text.log" \
	    announcement_text.txt
	svn copy --file ./announcement_text.log \
		svn+ssh://j_hoffmann@svn.gnu.org.ua/listings/trunk \
		svn+ssh://j_hoffmann@svn.gnu.org.ua/listings/tags/$(VERSION)
	rm announcement_text.log


## Documentation target
help::
	$(info Usage:)
	$(info )
	$(info make [all]	generates listings.sty and [all] the .pdf versions)
	$(info $(empty)		(user/developer) of the documentation)
	$(info )
	$(info make <file name>)
	$(info $(empty)		creates the corresponding file denoted by <file name>)
	$(info )
	$(info make help	shows this help)
	$(info )
	$(info make tests	performs a little test suite)
	$(info )
	$(info make clean	removes all intermediate files created by a LaTeX run)
	$(info )
	$(info make clean-results)
	$(info $(empty)		removes .cfg, .sty, and .pdf files)
	$(info )
	$(info make realclean)
	$(info $(empty)		performs clean and clean-results)
	$(info )
	$(info make tar-src)
	$(info $(empty)		generates a tarred version of the current directory)
	$(info )
	$(info make tar-dist)
	$(info $(empty)		generates a distributable version of the listings)
	$(info $(empty)		package)
	$(info )
	$(info make tagged-release)
	$(info $(empty)		creates a new tagged version of the package based on)
	$(info $(empty)		the contents of listings.version and announcement_text.txt)
	@echo ""					# prevents message "nothing to do ..."

### Makefile ends here ---


==> listings/README <==
Listings package

Copyright 1996--2004 Carsten Heinz (the package)
Copyright 1996--2007 individual authors (language drivers)
Copyright 2006--2007 Brooks Moses (continued maintenance)
Copyright 2013--2020 Jobst Hoffmann (continued maintenance)

Released under the LaTeX Project Public License 1.3c or later

The `listings' package is a source code printer for LaTeX.
You can typeset stand alone files as well as listings with
an environment similar to `verbatim' as well as you can
print code snippets using a command similar to \verb'.
Many parameters control the output and if your preferred
programming language isn't already supported, you can make
your own definition.


==> textgreek/README <==
This is the README file for the 'textgreek' package.

textgreek - text symbols for the Greek alphabet

SUMMARY

The LaTeX package textgreek provides NFSS text symbols for Greek
letters. This way an author can use Greek letters in text without
changing to math mode. The usual font selection commands---e.g.
\textbf---apply to these Greek letters as to usual text and the font
is upright in an upright environment. Further, hyperref can use these
symbols in PDF-strings such as PDF-bookmarks.

To produce the textgreek.sty file run

    latex textgreek.ins

FEEDBACK

Comments, suggestions, questions etc. are welcome. Send email to
leonard.michlmayr at gmail.com. (Preferably in German, English, or
Japanese)

LICENSE

Copyright 2010,2011 Leonard Michlmayr

This work may be distributed and/or modified under the
conditions of the LaTeX Project Public License, either version 1.3
of this license or (at your option) any later version.
The latest version of this license is in
  http://www.latex-project.org/lppl.txt
and version 1.3 or later is part of all distributions of LaTeX
version 2005/12/01 or later.

This work has the LPPL maintenance status `author-maintained'.
 
The Current Maintainer of this work is Leonard Michlmayr
<leonard.michlmayr at gmail.com>.

This work consists of the file textgreek.dtx
and the derived files textgreek.sty and textgreek.pdf


==> ts1/makets1.tex <==
\input fontinst.sty
\input textcomp.tex
\substitutesilent{n}{c}
\textcompfamily{ptm}{}
\textcompfamily{mbvx}{}
\textcompfamily{mntx}{}
\bye


==> ts1/october <==
Sebastian,

this reply took longer than expected, since the machine where I unpacked 
your package went down for about a week without prior announce.

First there are some omissions in the style file and/or the table:

\textblank    {'040}                               missing in the table
\textdivorced {'143} % divorced                    missing in both
\textdong     {'226} % Dong (currency of vietnam)  missing in both
\textpertenthousand {'230}                         missing in both
\textpilcrow  {'231}                               missing in both
\textbaht     {'232} % Baht (currency of thailand) missing in both


The 
\textshortequals 
should be taken from position {'055}, not as currently from {'177}:
The one at '177 is designed as a hanging hyphenchar, where '055 is non-
hanging (like usual hyphen).

I suggest to rename 
\textasciitilde {'176} to
\textlowtilde.
  In fact, the `ASCII tilde' is not defined in typographical terms, if it is 
high (like an accent) or low in its box. The dc fonts contain a high
`\textasciitilde'; the companion complement is by design low lying, 
therefore the suggested name \textlowtilde.

The 
\textbigcircle
is in fact that circle which is used by the \textcircled command. I 
therefore suggest to move the definition of \textcircled from OMSenc.def
to TS1. Here is the relevant snippet, adapted to TS1:

\DeclareTextCommand{\textcircled}{TS1}[1]{{%
   \ooalign{%
      \hfil \raise .07ex\hbox {\upshape#1}\hfil \crcr
      \char'117 % 
   }%
}}

Comment: Since the TS1 encoding provides oblique fonts (with oblique 
bigcircles!), the command \upshape can be removed.

The two tie accents are in fact meant to replace the definition of \t from
OMLenc.def (this is the only reference to OML in text mode). As a first step 
I suggest to use the `lowercase accent' everywhere, I'm just thinking on 
how to implement the choice of different accents according to the case of 
the accentee. This gives the following:

\DeclareTextAccent{\t}{TS1}{'032}

The definitions of 
\texttieaccentlowercase and \texttieaccentuppercase
can be dropped (both from the package and from the table).

[...]

Actually, here's what I'm suggesting for the accents designed for capital
letters:

There are commands like \capitalacute (you may want to add {text} to the 
names), defined in the following way:

%
% Acute accent for capitals
%
\DeclareTextAccentDefault{\capitalacute}{TS1}
\DeclareTextAccent{\capitalacute}{TS1}{'001}
%

This command can be used by the end user either directly or through 
definitions of the type

\DeclareTextCompositeCommand{\'}{T1}{X}{\capitalacute X}

None of the latter definitions should be provided by default, since they are 
probably rarely used.

Yours,
J"org Knappen.



==> verbatimbox/README <==
The style file verbatimbox has been created for the report writer's
convenience.

Do you need to include blocks of verbatim text inside figures, tables or
footnotes?  The verbatim environment is not compatible with some of
these other environments.  But now, the verbbox environment allows you
to input verbatim text and store it in a LaTeX box.  That box then
becomes generally usable in all other LaTeX environments, and can be
simply recalled.

This style therefore allows for a greater use of the verbatim
environment within other LaTeX constructs where verbatim was previously
inaccessible.

Input to the verbatim box can either be as text typed into the verbbox
or myverbbox environments, or else as the contents of a file, provided
as an argument to the \verbfilebox command.  In either case, an optional
argument may be provided to modify the text appearance, for example, by
changing the font size of the verbatim text placed into the box.

The \addvbuffer command, while supporting this package, also provides a
flexible way to add vertical buffer space above and below most LaTeX
objects, which can be handy in a variety of applications.

						-Steven Segletes


==> was/README <==
============================================================

          The contents of the CTAN directory "was"

============================================================
                                              Walter Schmidt
                                         w.a.schmidt@gmx.net


fixmath:  A LaTeX package to provide italic uppercase Greek
  letters in math and an additional bold italic math
  alphabet \mathbold; to be used with the default CM math
  fonts.

icomma:  With ordinary LaTeX, the comma cannot be used as a
  decimal separator in math mode, because it is treated as a
  punctuation character and LaTeX adds some extra space
  after it.  This can be overcome by defining an
  `intelligent' comma, which adds the space only, if the
  next input character is actually a blank.  In contrast to
  other known solutions, the LaTeX package icomma.sty does
  not rely on the particular encoding of the CM math fonts,
  and it works with decimal numbers of arbitrary length.

upgreek:  A LaTeX macro package to provide the upright Greek
  letters from the Euler or Adobe Symbol fonts as additional
  math symbols, with proper scaling in super- and
  subscripts.
  
gensymb:  This LaTeX package provides generic commands
  \degree, \celsius, \perthousand, \micro and \ohm, which
  work both in text and math mode.  The package should
  co-operate flawlessly with the well-known units.sty.
  Various means are provided to fake the symbols or take
  them from external symbol fonts, if they are not available
  in the default fonts used in the document.  The package
  makes optionally use of upgreek.sty.

The style files can be unpacked by running the particular
installation script (.ins) through LaTeX.  The files will 
be created immediately in the appropriate TDS directory
tex/latex/was, if this directory exists and the DOCSTRIP
tool is properly configured -- otherwise they are written
into the current directory.

The documentation of a package can be generated by running
the particular .dtx file through LaTeX.

==finis


==> xcolor/ChangeLog <==
Package `xcolor' by Dr. Uwe Kern
(xcolor at ukern dot de)

History
=======

2016/05/11 v2.12
* New features:
    - \nopagecolor command as introduced in `color' v1.1a
      (example added to xcolor3.tex);
    - `luatex' driver option (code provided by DPC) to fix
      incompatibilities due to changes in new LuaTeX version.
* Bugfixes:
    - possible name conflict by \XC@ifxcase call;
    - incorrect internal \@hex@@Hex macro.

2007/01/21 v2.11
* New features:
    - color names `lime' and `teal' added to the set of predefined
      colors.
* Bugfix:
    - incorrect \XC@strip@comma call within `hyperref'-related options.

2006/11/28 v2.10
* New features:
    - `fixinclude' option prevents dvips from explicitly resetting
      current color to `black' before actually inserting an .eps file
      via \color{red}\includegraphics{foo}.
* Changes:
    - \colorbox and \fcolorbox made robust;
    - obsolete package option `pst' removed;
    - several changes to internal macros.
* Bugfixes:
    - incorrect processing of cmyk-type current color `.'.

2005/12/21 v2.09
* New features:
    - \definecolor and \color now accept space-separated color
      specifications, e.g., \color[rgb]{1 .5 0};
    - experimental `xcdraw' option extended to `pdftex' and `dvipdfm'
      drivers.
* Changes:
    - test file xcolor2.tex made compatible with recent changes in
      `pstricks';
    - test file xcolor3.tex extended;
    - driver test file xcolor4.tex extended to demonstrate the different
      frame drawing approaches;
    - more efficient implementation of driver-specific code.

2005/11/25 v2.08
* New features:
    - more flexibility for \fcolorbox arguments, e.g.,
      \fcolorbox[gray]{0.5}[wave]{580}{test};
    - \boxframe returns a frame of given dimensions;
    - new implementation of \f(rame)box and \fcolorbox as an extension
      of bug report latex/3655 to reduce pixel positioning errors in
      output devices;
    - `kernelfbox' option for those who prefer the previous \f(rame)box
      approach;
    - experimental `xcdraw' option uses PostScript commands to draw
      frames and color boxes in case of `dvips'.
* Bugfixes:
    - insufficient expression type detection within \colorlet;
    - wrong calculation in the unit interval reduction for negative
      integers (affecting color series and extended color expressions).

2005/11/12 v2.07
* New features:
    - color model `Hsb' allows to specify hue in degrees;
    - color model `tHsb' (`tuned Hsb') for user-defined hue
      configuration on color wheels;
    - easy generation of color harmonies derived from `Hsb' or `tHsb'
      color wheels, e.g., \color{red>wheel,1,12} yields an `analogous'
      color to `red' on a 12-spoke wheel;
    - additional 317 predefined color names according to rgb.txt, which
      is part of Unix/X11 distributions;
    - `svgnames' option extended by 4 colors taken from rgb.txt;
    - enhanced syntax for immediate conversion, e.g.,
      \definecolor{foo}{rgb:gray}{0.3} or \color[rgb:wave]{478};
    - \@ifundefinedcolor and \@ifundefinedmodel commands.
* Changes:
    - enhanced documentation;
    - several changes to internal macros.
* Bugfixes:
    - wrong calculation of color series components in some cases of
      negative step parameters.

2005/10/15 v2.06
* New features:
    - color model `wave' for (approximate) visualisation of light
      wavelengths, still somewhat experimental;
    - pseudo-model `ps' for colors defined by literal PostScript code
      in conjunction with `pstricks and `dvips'; an illustrative
      example for a gamma-correction approach is given in xcolor2.tex;
    - \substitutecolormodel command for replacement of missing or
      faulty driver-specific color models;
    - improved detection and handling of driver-specific color models;
    - `dvipdfmx' and `xetex' options to support these drivers;
    - generic driver test file xcolor4.tex.
* Changes:
    - \XC@strip@comma doesn't generate a trailing space anymore, which
      improves also the output of the `testcolors' environment.

2005/09/30 v2.05
* New features:
    - `testcolors' environment helps to test colors in different models,
      showing both the visual result and the model-specific parameters;
    - \extractcolorspecs puts model/color specification into two
      separate commands, as opposed to \extractcolorspec;
    - color names `pink' and `olive' added to the set of predefined
      colors.
* Bugfixes:
    - \definecolor{foo}{named}{bar} did not work in v2.04.

2005/09/23 v2.04
* New features:
    - preparation for usage of additional - driver-provided - color
      models;
    - `pstricks' users may now specify explicit color parameters within
      \psset and related commands, e.g., \psset{linecolor=[rgb]{1,0,0}};
      an illustrative example is given in xcolor2.tex.
* Changes:
    - color model names sanitized (i.e., turned to catcode 12)
      throughout the package;
    - \@namelet command deprecated because of name clash with
      `memoir' - please use \XC@let@cc instead
      (more \XC@let@.. commands are available as well);
    - simplified color conversion code by using the new \XC@ifxcase
      command;
    - some minor changes to internal macros.

2005/06/06 v2.03
* New features:
    - `fixpdftex' option loads `pdfcolmk' package in order to improve
      pdfTeX's color behaviour during page breaks.
* Changes:
    - some minor changes to internal macros.
* Bugfixes:
    - due to an incorrect \if statement within \XC@info, \colorlet
      caused trouble whenever its second argument started with two
      identical letters, e.g., \colorlet{rab}{oof};
    - argument processing of \XC@getcolor caused incompatibility with
      `msc' package;
    - `prologue' option caused incompatibility with `preview' package.

2005/03/24 v2.02
* New features:
    - \aftergroupedef command to reproduce \aftergroupdef's behaviour
      prior to v2.01;
    - xcolor's homepage www.ukern.de/tex/xcolor.html now provides also
      a ready-to-run TDS-compliant archive containing all required
      files.
* Changes:
    - \rowcolors and friends are solely enabled by the `table' option;
    - \@ifxempty changed back to more robust variant of v2.00.
* Bugfixes:
    - \psset{linecolor=\ifcase\foo red\or green\or blue\fi} did not work
      with `pstricks' (error introduced in v2.01).

2005/03/15 v2.01
* New features:
    - `prologue' option for comprehensive `named' color support in
      conjunction with `dvips': on-the-fly generation of PostScript
      prologue files with all color definitions, ready for dvips
      inclusion and/or post-processing with device-specific parameters
      (e.g., spot colors);
    - dvips prologue file xcolor.pro to support additional `named'
      colors;
    - \colorlet may now also be used to create named colors from
      arbitrary color expressions;
    - enhanced color definition syntax to allow for target-model
      specific color parameters, e.g.,
      \definecolor{red}{rgb/cmyk}{1,0,0/0,1,1,0}, facilitating the
      usage of tailor-made colors both for displays and printers;
    - `deferred definition' of colors: \preparecolor and
      \definecolors enable decoupling of color specification and control
      sequence generation, especially useful (= memory saving) for large
      lists of colors, of which only a few names are actually used;
    - `dvipsnames*' and `svgnames*' options to support deferred
      definition.
* Changes:
    - higher accuracy: most complement calculations are now exact for
      all 5-digit decimals;
    - \rangeRGB and similar variables may now be changed at any point
      in a document;
    - \aftergroupdef now performs only a first-level expansion of its
      code argument;
    - \XCfileversion and similar internal constants removed from .sty
      and .def files;
    - improved memory management (reduced generation of `multiletter
      control sequences' by \@ifundefined tests);
    - several internal macros improved and/or renamed.
* Bugfixes:
    - \XC@getcolor could cause unwanted spaces when \psset was used
      inside |pspicture| environments (`pstricks');
    - arithmetic overflow could happen when too many decimal digits
      were used within color parameters, e.g., as a result of `fp'
      calculations.

2004/07/04 v2.00
* New features:
    - extended functionality for color expressions: mix colors like a
      painter;
    - support for color blending: specify color mix expressions that
      are being blended with every displayed color;
    - \xglobal command for selective control of globality for color
      definitions, blends, and masks;
    - multiple step operations (e.g., \color{foo!!+++}) and access to
      individual members (e.g., \color{foo!![7]}) in color series;
    - \providecolor command to define only non-existent colors;
    - \definecolorset and \providecolorset commands to facilitate the
      construction of color sets with common underlying color model;
    - additional 147 predefined color names according to SVG 1.1
      specification;
    - `xpdfborder' key for setting the width of hyperlink borders in a
      more driver-independent way if `dvips' is used.
* Changes:
    - `color' package now completely integrated within `xcolor';
    - `override', `usenames', `nodvipsnames' options and \xdefinecolor
      command no longer needed;
    - `dvips' and `dvipsnames' options now independent of each other;
    - \tracingcolors's behaviour changed to make it more versatile and
      reduce log file size in standard cases;
    - \rdivide's syntax made more flexible (divide by numbers and/or
      dimensions);
    - code restructured, some internal commands renamed;
    - documentation rearranged and enhanced.
* Bugfixes:
    - \definecolor{foo}{named}{bar} did not work (error introduced in
      v1.11);
    - more robust behaviour of conditionals within `pstricks'
      key-values.

2004/05/09 v1.11
* New features:
    - switch \ifglobalcolors to control whether color definitions are
      global or local;
    - option `hyperref' provides color expression support for the
      border colors of hyperlinks, e.g.,
      \hypersetup{xurlbordercolor=red!50!yellow};
    - internal hooks \XC@bcolor, \XC@mcolor, and \XC@ecolor for
      additional code that has to be executed immediately before/after
      the current color is being displayed.
* Changes:
    - \XC@logcolor renamed to \XC@display, which is now the core color
      display command;
    - improved interface to `pstricks'.

2004/03/27 v1.10
* New features:
    - support for `named' model;
    - support for `dvips' colors
      (may now be used within color expressions);
    - internal representation of `ordinary' and `named' colors merged
      into unified data structure;
    - allow multiple `-' signs at the beginning of color expressions.
* Bugfixes:
    - commands like \color[named]{foo} caused errors when color masking
      or target model conversion were active;
    - incompatibility with `soul' package: commands \hl, \ul, etc.
      could yield unexpected results.
* Documentation:
    - added formula for general color expressions;
    - enhanced text and index;
    - removed dependence of index generation on local configuration
      file.

2004/02/16 v1.09
* New features:
    - color model `HTML', a 24-bit hexadecimal `RGB' variant;
      allows to specify colors like \color[HTML]{AFFE90};
    - color names `orange', `violet', `purple', and `brown' added to
      the set of predefined colors.
* New xcolor homepage: www.ukern.de/tex/xcolor.html
* Bugfix: \xdefinecolor sometimes did not normalise its parameters.
* Changes:
    - slight improvements of the documentation;
    - example file xcolor1.tex reorganised and abridged.

2004/02/04 v1.08
* New commands/features:
    - \selectcolormodel to change the target model within a document;
    - \adjustUCRBG to fine-tune undercolor-removal and
      black-generation during conversion to `cmyk'.
* Bugfix: color expressions did not work correctly in connection with
  active `!' character, e.g., in case of \usepackage[frenchb]{babel}.
* Code re-organisation:
    - \XC@xdefinecolor merged into \xdefinecolor, making the first
      command obsolete;
    - several internal commands improved/streamlined.

2004/01/20 v1.07
* New feature: support for color masking and color separation.
* New commands:
    - \rmultiply to multiply a dimension register by a real number;
    - \xcolorcmd to pass commands that are to be executed at the end
      of the package.
* Changes:
    - more consistent color handling: extended colors now always take
      precedence over standard colors;
    - several commands improved by using code from the LaTeX kernel.
* Documentation: some minor changes.
* Example files: additional `pstricks' examples (file xcolor2.tex).

2003/12/15 v1.06
* New feature: extended color expressions, allowing for cascaded mix
  operations, e.g., \color{red!30!green!40!blue}.
* Documentation: new section on color expressions.
* Bugfix: color series stepping did not work correctly within
  non-displaying commands like \extractcolorspec{foo!!+}
  (this bug was introduced in v1.05).
* Renamed commands: \ukfileversion and similar internal constants
  renamed to \XCfileversion etc.
* Removed commands: \ifXCpst and \ifXCtable made obsolete by a simple
  trick.

2003/11/21 v1.05
* Bugfixes:
    - package option `hideerrors' should now work as expected;
    - usage of `.' in the first color expression in a document caused
      an error due to incorrect initialisation.
* Code re-organisation: \extractcolorspec now uses \XC@splitcolor,
  making \XC@extract obsolete.

2003/11/09 v1.04
* New feature: easy access to current color within color expressions.
* New option: `override' to replace \definecolor by \xdefinecolor.
* New command: \tracingcolors for logging color-specific information.

2003/09/21 v1.03
* Change: bypass strange behaviour of some drivers.
* New feature: driver-sharing with `hyperref'.

2003/09/19 v1.02
* Change: \extractcolorspec and \colorlet now also accept color series
  as arguments.

2003/09/15 v1.01
* New feature: \definecolorseries and friends.
* Documentation: removed some `doc'-related side-effects.
* Code re-organisation: all calculation-related tools put to one place.
* Bugfixes:
    - \@rdivide: added \relax to fix problem with negative numerators;
    - \rowc@l@rs: replaced \@ifempty by \@ifxempty.

2003/09/09 v1.00
* First published release.


==> xcolor/README <==
Package `xcolor' by Dr. Uwe Kern
(xcolor at ukern dot de)

v2.12 (2016/05/11)

`xcolor' provides easy driver-independent access to several kinds of
colors, tints, shades, tones, and mixes of arbitrary colors by means of
color expressions like \color{red!50!green!20!blue}.
It allows to select a document-wide target color model and offers tools
for automatic color schemes, conversion between nine color models,
alternating table row colors, color blending and masking, color
separation, and color wheel calculations.

Installation instructions
=========================

Extract all package files:
  `latex xcolor.ins'

Put the generated files to their respective locations
within the TeX installation:
  *.sty -> /tex/latex/xcolor/
  *.def -> /tex/latex/xcolor/
  *.pro -> /dvips/xcolor/

Create the documentation:
  `latex xcolor.dtx'
  `latex xcolor.dtx'
  `makeindex -s gind.ist xcolor.idx'
  `latex xcolor.dtx'
  `latex xcolor.dtx'

Run the test files (N=1,2,...):
  `latex xcolorN.tex'
  `latex xcolorN.tex'

Notes
=====

- `xcolor1.tex' should run with both LaTeX and pdfLaTeX, it yields a
  50-page document with several systematic color conversion examples
- `xcolor2.tex' is a 3-page `pstricks' example document that won't run
  with pdfLaTeX
- `xcolor3.tex' is a 2-page example for demonstrating several display
  and logging facilities
- `xcolor4.tex' is a 1-page driver test file;
  uncomment the relevant code line in the header and run it with the
  appropriate program, e.g., `latex xcolor4' or any other processor;
  apply any desired post-processing like dvips, dvipdfm, etc.
- If the file `xcolor.ins' is missing, run `latex xcolor.dtx' once
  and quit the LaTeX compiler as soon as the first error message
  appears.

History
=======

See file `ChangeLog'.

